Flexible, Decentralized Access Control for Smart Buildings with Smart Contracts

Large commercial buildings are complex cyber-physical systems containing expensive and critical equipment that ensure the safety and comfort of their numerous occupants. Yet occupant and visitor access to spaces and equipment within these buildings are still managed through unsystematic, inefficient, and human-intensive processes. As a standard practice, long-term building occupants are given access privileges to rooms and equipment based on their organizational roles, while visitors have to be escorted by their hosts. This approach is conservative and inflexible. In this paper, we describe a methodology that can flexibly and securely manage building access privileges for long-term occupants and short-term visitors alike, taking into account the risk associated with accessing each space within the building. Our methodology relies on blockchain smart contracts to describe, grant, audit, and revoke fine-grained permissions for building occupants and visitors, in a decentralized fashion. The smart contracts are specified through a process that leverages the information compiled from Brick and BOT models of the building. We illustrate the proposed method through a typical application scenario in the context of a real office building and argue that it can greatly reduce the administration overhead, while, at the same time, providing fine-grained, auditable access control.

==> illustrative-scenario.tex <==
%-----------------------------------------
\section{An Illustrative Application Scenario}\label{sec:scenario}
%-----------------------------------------
Consider a simple application scenario which involves inviting a group of individuals 
to a meeting that takes place in a specific room of an office building.
We describe how our access-control methodology, presented in the next section, 
would facilitate this application

The process starts with a calendar invitation created by the meeting host, 
listing the individuals invited (their names and email addresses), 
the room where the meeting is to be held, and the time when it is to take place. 
The first step is to examine whether the invited individuals are known to the access-control service: 
if not, new entities need to be created to represent their credentials (see Section~\ref{method3}). 
Next, the possible paths in the building to reach the meeting room are computed and presented to the meeting host (see Section~\ref{method1})\footnote{Here 
we only consider the problem of indoor path planning, from a main building door to the meeting room,
but our methodology can be extended to 
the overall problem of planning a path from each individual's location, 
taking into account their route preferences and parking needs, 
as long as the relevant information is captured by some model.}.
Each of the possible indoor paths is presented to the meeting host with a cost that represents its sensitivity (see Section~\ref{method2}) 
and the building elements (equipment, sensors, and setpoints) that contribute to it. 
The host reviews the possible paths and selects the preferred one (possibly the one that has the lowest cost).

The selected path is then transformed into a smart contract (see Section~\ref{method3}), 
where the meeting host delegates each invitee with the necessary privileges to access the various doorways on the path, 
and a personalized QR code (akin to a boarding pass) is generated to represent each contract. 
These QR codes are shared with each participant along with the calendar invitation.

Before the meeting occurs, each meeting participant arrives to the building and uses the QR code to open every door on the path from the building entrance to the designated meeting room.
Each QR code scan invokes a request to the Ethereum ledger (see Section~\ref{method4}) to check whether 
the bearer is authorized to access the corresponding door at the present time and in a specific order.
If the meeting host has access to these rooms and had authorized the meeting participants to access these rooms before the meeting,
the access is verified and a signal is sent to the electric door strike to open the door.
The process repeats for each door along the path.
We explain our methodology in the following.

==> sensors.tex <==
brick:AHU_Filter_Pressure_Sensor
brick:AHU_HT_WHL_C_Sensor
brick:AHU_HT_WHL_S_Sensor
brick:AHU_LVL0_EOL_Pressure_Sensor
brick:AHU_Mixed_Air_Damper_Sensor
brick:AHU_Mixed_Air_Flow_Sensor
brick:AHU_Mixed_Air_Temperature_Sensor
brick:AHU_Outside_Air_Flow_Sensor
brick:Damper_Sensor
brick:Differential_Pressure_Sensor
brick:End_of_Line_Pressure_Sensor
brick:Entering_Air_Temperature_Sensor
brick:Exhaust_Fan_Flow_Sensor
brick:Exhaust_Fan_Speed_Sensor
brick:FZ_Sensor
brick:Flow_Sensor
brick:Glycol_Feed_Unit_DP_Sensor
brick:Glycol_Feed_Unit_EXP_Pressure_Sensor
brick:Glycol_Feed_Unit_GWRT_Temperature_Sensor
brick:Glycol_Feed_Unit_P1A_C_Sensor
brick:Glycol_Feed_Unit_P1A_S_Sensor
brick:Glycol_Feed_Unit_P1B_C_Sensor
brick:Glycol_Feed_Unit_P1B_S_Sensor
brick:Glycol_Feed_Unit_Valve_Sensor

brick:Preheating_Coil_Temperature_Sensor
brick:Preheating_Coil_Valve_Sensor
brick:Pressure_Sensor
brick:Reheat_Coil_Valve_Sensor
brick:Return_Air_Temperature_Sensor
brick:Room_Temperature_Poll_Sensor
brick:Room_Temperature_Sensor
brick:Sensor
brick:Speed_Sensor
brick:Status_Sensor
brick:Supply_Air_Temperature_Sensor
brick:Supply_Fan_Flow_Sensor
brick:Supply_Fan_Speed_Sensor
brick:Supply_Fan_Status_Sensor
brick:Telecom_Room_Temperature_Sensor
brick:Temperature_Sensor
brick:VAV_Flow_Sensor


brick:Air_Flow_Setpoint
brick:Building_Static_Pressure_Setpoint
brick:Bypass_Setpoint
brick:Chiller_Valve_Pull_Setpoint
brick:Damper_Close_Setpoint
brick:Damper_Open_Setpoint
brick:End_of_Line_Setpoint
brick:Entering_Air_Dam_Setpoint
brick:Exhaust_Fan_Status_Setpoint
brick:Glycol_Feed_Unit_DP_Setpoint
brick:Glycol_Feed_Unit_GWST_Setpoint
brick:Glycol_Feed_Unit_HWST_Setpoint
brick:Glycol_Feed_Unit_P1A_C_Setpoint
brick:Glycol_Feed_Unit_P1B_C_Setpoint
brick:Radiator_Valve_Setpoint
brick:Room_Temperature_Setpoint
brick:Room_Temperature_Setpoint;
brick:Setpoint
brick:Supply_Air_Temperature_Setpoint
brick:Supply_Fan_Variable_Frequency_Drive_Setpoint
brick:VAV_Flow_Setpoint
brick:Variable_Frequency_Drive_Setpoint
